Emergent Features in $U(N) \times U(\tilde{N})$ Bi-adjoint Cubic Theory

This work investigates the role of the $U(N) \times U(\tilde{N})$ global symmetry in tree-level scattering amplitudes of the bi-adjoint $\phi^3$ theory from three perspectives: combinatorics, correlation functions, and a massive extension of the CHY formalism. We derive a planar scattering potential whose extrema reproduce Dolan and Goddard's massive scattering equations, providing physical intuition of the construction. This potential enables the counting of kinematic invariants via maximally symmetric Ferrers shapes, and it is expressed in terms of conformally invariant cross-ratios. We find that the $U(1)$ decoupling identity provides a physical interpretation of two different Catalan recursion relations, and also reveals an interplay between Catalan and Narayana numbers in the $U(1)$ splitting. Finally, we construct correlation functions for a fixed particle ordering using the CHY formalism, offering new insights into the dynamics of such amplitude structures. We derive a closed form expression of the reduced number of solutions for this set-up, as well as an off-shell scattering potential.

==> style_files/PSI_front_matter_compilation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT/DELETE THIS FILE  %%
%% (for use in book compilation) %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\headheight}{15pt} 

% The heading on the front page
\chapter*{\essaytitle} 

\vspace{-0.5cm}
\centerline{\textbf{\yourname}} 
\vspace{0.3cm}
\centerline{Supervisor: \yoursupervisor} 
\vspace{0.5cm} 


